Visual Editing with LLM-based Tool Chaining: An Efficient Distillation Approach for Real-Time Applications

We present a practical distillation approach to fine-tune LLMs for invoking tools in real-time applications. We focus on visual editing tasks; specifically, we modify images and videos by interpreting user stylistic requests, specified in natural language ("golden hour"), using an LLM to select the appropriate tools and their parameters to achieve the desired visual effect. We found that proprietary LLMs such as GPT-3.5-Turbo show potential in this task, but their high cost and latency make them unsuitable for real-time applications. In our approach, we fine-tune a (smaller) student LLM with guidance from a (larger) teacher LLM and behavioral signals. We introduce offline metrics to evaluate student LLMs. Both online and offline experiments show that our student models manage to match the performance of our teacher model (GPT-3.5-Turbo), significantly reducing costs and latency. Lastly, we show that fine-tuning was improved by 25% in low-data regimes using augmentation.

==> latex/4_experiments/parameters_evaluation.tex <==



% For our offline evaluation experiments (see Section~\ref{subsec:offline_evaluation} -- Intrinsic Parameters Evaluation Metrics), we used our test set from our data collection for fine-tuning phase 
% (see Section~\ref{subsec:data_collection}) of 1,000 unique user intents resulting in 3,000 samples (as each intent requires the student LLM to predict parameters on three different tools).



%flan-t5 all data prod run
% Prod run: colorful-dragonfly
% avg: 0.72
% filter_fr1_final:0.74
% filter_fr1_quality:0.71
% filter_fr1_usability:0.78
% filter_fr3_final:0.79
% filter_fr3_quality:0.72
% filter_fr3_usability:0.88
% filter_fr5_final:0.85
% filter_fr5_quality:0.82
% filter_fr5_usability:0.89

% selective_adjust_fr1_final:0.70
% selective_adjust_fr1_quality:0.65
% selective_adjust_fr1_usability:0.76
% selective_adjust_fr3_final:0.75
% selective_adjust_fr3_quality:0.66
% selective_adjust_fr3_usability:0.87
% selective_adjust_fr5_final:0.79
% selective_adjust_fr5_quality:0.71
% selective_adjust_fr5_usability:0.90

% adjust_fr1_final:0.72
% adjust_fr1_quality:0.57
% adjust_fr1_usability:0.95
% adjust_fr3_final:0.76
% adjust_fr3_quality:0.61
% adjust_fr3_usability:0.99
% adjust_fr5_final:0.80
% adjust_fr5_quality:0.68
% adjust_fr5_usability:0.99




% dramatic-stoat: random sample 1/8 without aug
% avg: 0.52
% filter_fr1_final:0.66
% filter_fr1_quality:0.57
% filter_fr1_usability:0.79
% filter_fr3_final:0.68
% filter_fr3_quality:0.56
% filter_fr3_usability:0.87
% filter_fr5_final:0.68
% filter_fr5_quality:0.56
% filter_fr5_usability:0.86

% selective_adjust_fr1_final:0.28
% selective_adjust_fr1_quality:0.19
% selective_adjust_fr1_usability:0.61
% selective_adjust_fr3_final:0.31
% selective_adjust_fr3_quality:0.2
% selective_adjust_fr3_usability:0.73
% selective_adjust_fr5_final:0.34
% selective_adjust_fr5_quality:0.22
% selective_adjust_fr5_usability:0.72

% adjust_fr1_final:0.62
% adjust_fr1_quality:0.46
% adjust_fr1_usability:0.96
% adjust_fr3_final:0.61
% adjust_fr3_quality:0.44
% adjust_fr3_usability:0.99
% adjust_fr5_final:0.71
% adjust_fr5_quality:0.55
% adjust_fr5_usability:0.98


% ethereal-hippo: random sample 1/8 with aug
% avg: 0.65
% filter_fr1_final:0.72
% filter_fr1_quality:0.64
% filter_fr1_usability:0.82
% filter_fr3_final:0.74
% filter_fr3_quality:0.63
% filter_fr3_usability:0.90
% filter_fr5_final:0.74
% filter_fr5_quality:0.62
% filter_fr5_usability:0.91
% adjust_fr1_final:0.64
% adjust_fr1_quality:0.49
% adjust_fr1_usability:0.95
% adjust_fr3_final:0.65
% adjust_fr3_quality:0.48
% adjust_fr3_usability:0.99
% adjust_fr5_final:0.69
% adjust_fr5_quality:0.54
% adjust_fr5_usability:0.98
% selective_adjust_fr1_final:0.59
% selective_adjust_fr1_quality:0.50
% selective_adjust_fr1_usability:0.70
% selective_adjust_fr3_final:0.60
% selective_adjust_fr3_quality:0.49
% selective_adjust_fr3_usability:0.78
% selective_adjust_fr5_final:0.63
% selective_adjust_fr5_quality:0.53
% selective_adjust_fr5_usability:0.77



% sturdy-frigatebird (1/4 random sample no aug)
% avg: 0.60
% filter_fr1_final:0.68
% filter_fr1_quality:0.58
% filter_fr1_usability:0.81
% filter_fr3_final:0.71
% filter_fr3_quality:0.59
% filter_fr3_usability:0.89
% filter_fr5_final:0.75
% filter_fr5_quality:0.65
% filter_fr5_usability:0.89

% selective_adjust_fr1_final:0.47
% selective_adjust_fr1_quality:0.41
% selective_adjust_fr1_usability:0.55
% selective_adjust_fr3_final:0.48
% selective_adjust_fr3_quality:0.40
% selective_adjust_fr3_usability:0.58
% selective_adjust_fr5_final:0.57
% selective_adjust_fr5_quality:0.55
% selective_adjust_fr5_usability:0.6

% adjust_fr1_final:0.67
% adjust_fr1_quality:0.51
% adjust_fr1_usability:0.96
% adjust_fr3_final:0.67
% adjust_fr3_quality:0.50
% adjust_fr3_usability:0.99
% adjust_fr5_final:0.71
% adjust_fr5_quality:0.55
% adjust_fr5_usability:0.99


% groovy-hamster (1/4 random sample with aug)
% avg: 0.66
% filter_fr1_final:0.70
% filter_fr1_quality:0.64
% filter_fr1_usability:0.78
% filter_fr3_final:0.71
% filter_fr3_quality:0.60
% filter_fr3_usability:0.85
% filter_fr5_final:0.72
% filter_fr5_quality:0.64
% filter_fr5_usability:0.82

% selective_adjust_fr1_final:0.59
% selective_adjust_fr1_quality:0.50
% selective_adjust_fr1_usability:0.72
% selective_adjust_fr3_final:0.63
% selective_adjust_fr3_quality:0.50
% selective_adjust_fr3_usability:0.85
% selective_adjust_fr5_final:0.70
% selective_adjust_fr5_quality:0.59
% selective_adjust_fr5_usability:0.86

% adjust_fr1_final:0.69
% adjust_fr1_quality:0.54
% adjust_fr1_usability:0.95
% adjust_fr3_final:0.71
% adjust_fr3_quality:0.55
% adjust_fr3_usability:0.99
% adjust_fr5_final:0.71
% adjust_fr5_quality:0.55
% adjust_fr5_usability:0.99






% denim-inchworm  (1/2 random sample no aug)
% avg: 0.68
% filter_fr1_final:0.71
% filter_fr1_quality:0.63
% filter_fr1_usability:0.81
% filter_fr3_final:0.75
% filter_fr3_quality:0.64
% filter_fr3_usability:0.90
% filter_fr5_final:0.79
% filter_fr5_quality:0.69
% filter_fr5_usability:0.92

% selective_adjust_fr1_final:0.64
% selective_adjust_fr1_quality:0.58
% selective_adjust_fr1_usability:0.71
% selective_adjust_fr3_final:0.66
% selective_adjust_fr3_quality:0.56
% selective_adjust_fr3_usability:0.82
% selective_adjust_fr5_final:0.68
% selective_adjust_fr5_quality:0.57
% selective_adjust_fr5_usability:0.86

% adjust_fr1_final:0.69
% adjust_fr1_quality:0.54
% adjust_fr1_usability:0.95
% adjust_fr3_final:0.69
% adjust_fr3_quality:0.53
% adjust_fr3_usability:0.98
% adjust_fr5_final:0.73
% adjust_fr5_quality:0.58
% adjust_fr5_usability:0.99


% flying-hyena (1/2 random sample with aug)
% avg: 0.70

% filter_fr1_final:0.74
% filter_fr1_quality:0.67
% filter_fr1_usability:0.82
% filter_fr3_final:0.77
% filter_fr3_quality:0.67
% filter_fr3_usability:0.91
% filter_fr5_final:0.81
% filter_fr5_quality:0.72
% filter_fr5_usability:0.94

% selective_adjust_fr1_final:0.66
% selective_adjust_fr1_quality:0.62
% selective_adjust_fr1_usability:0.70
% selective_adjust_fr3_final:0.68
% selective_adjust_fr3_quality:0.61
% selective_adjust_fr3_usability:0.78
% selective_adjust_fr5_final:0.71
% selective_adjust_fr5_quality:0.63
% selective_adjust_fr5_usability:0.82

% adjust_fr1_final:0.71
% adjust_fr1_quality:0.57
% adjust_fr1_usability:0.95
% adjust_fr3_final:0.73
% adjust_fr3_quality:0.58
% adjust_fr3_usability:0.99
% adjust_fr5_final:0.77
% adjust_fr5_quality:0.63
% adjust_fr5_usability:0.99



% \noindent\textbf{Dataset.} 
% Our dataset for fine-tuning is generated by including responses of ChatGPT (one-shot prompt) for the different tools, to different user's requests received in the application (Section \ref{subsec:data_generation}).
% These samples are then filtered by including only responses which led to \emph{export} -- which means the user chose to use the generated output (Section \ref{subsec:data_filtering}).

% Specifically, we filtered data for every tool by taking samples that passed two thresholds: (1) export rate(\%) and (2) user's request count. 
% This way we take only samples with responses achieving exports (we found that 80\% of the original data does not include exports at all), for repeated user's requests.
% Then, given a set of different responses for the same user's request which pass the export rate threshold, we take the one with the maximum export rate.
% See Appendix for full details of the threshold's values for each tool.

% Table~\ref{tab:dataset_distribution} shows statistics on the size of data for fine-tuning. 
% The samples include distinct user request as an input, and the parameter's values and optional free text reasoning (CoT) as an output. 
% In training we use disjoint sets of samples for each tool. In test, we use the same set of 100 samples.
% As can be seen, \emph{adjust} and \emph{filter} are mostly should be used, and \emph{selective adjust} is expected to be used around half of the times.




% \begin{table}[!t]
%     \centering
%     \footnotesize % Smaller font size for compactness
%     \begin{tabular}{l cc cc cc}
%         \toprule
%         \textbf{Data} & \multicolumn{2}{c}{\textbf{Adjust}} & \multicolumn{2}{c}{\textbf{Selective Adjust}} & \multicolumn{2}{c}{\textbf{Filter}} \\
%         & Used & Total & Used & Total & Used & Total \\
%         \midrule
%         Train & 648 & 661 & 364 & 604 & 584 & 681 \\
%         \midrule
%         Test & 98 & 100 & 43 & 100 & 95 & 100 \\
%         \bottomrule
%     \end{tabular}
%     \caption{Data distribution for fine-tuning: for each tool, we have samples with distinct user requests as an input, and the parameter's values and optional free text reasoning (CoT) as an output. Training involves separate sets for each tool, around 600 samples per tool (see ``Total'' column); testing assesses a uniform set of 100 requests. \emph{selective adjust} expected to be used in half of cases, \emph{adjust} and \emph{filter} are mostly used (see ``Used'' column).}
%     \label{tab:dataset_distribution}
% \end{table}






    






% \noindent\textbf{Baselines.}
% We fine-tuned different  \emph{state-of-the-art LLMs}, both \emph{sequence-to-sequence} and \emph{auto-regressive} models. 
% For our \emph{auto-regressive} model baseline, we evaluated LLaMA 2 \cite{touvron2023llama2} with 7B parameters.
% In order to reduce the number of trainable parameters, and consequently the GPU memory requirements, 
% we trained LLaMA 2 with Parameter Efficient Training (PEFT), using Low Rank Adaptations (LoRA)
% \cite{hu2021lora}. 

% For our \emph{sequence-to-sequence} baselines, we evaluated different sizes of Flan-T5 models \cite{chung2022scaling}
% , which are smaller than LLaMA 2 (from Flan-T5-small with 80M parameters to Flan-T5-xl with 3B parameters).
% Our aim in exploring smaller LLMs is to find models that keep high quality results, in lower latency and lower cost of GPU.

% We train one model on the three different tools, selecting the checkpoint which maximizes performance overall.
% Training one model for all tools, rather than one per tool, involved trade-offs. It led to a minor reduction in accuracy, 
% as we do not select the best checkpoint per tool anymore, and limited flexibility in model size variation (e.g., if one of the tools is simpler, we can choose a smaller model for fine-tuning on this tool). 
% However, we decided to choose this approach as it offers us a scalable and low cost solution (in terms of GPUs).

% See Appendix for full details of model's parameters we used during training and inference.

% \noindent\textbf{Evaluation metrics.}
% We evaluate the models on the two elements of the task. (1) \emph{Usability:} the model's ability to decide correctly whether to use a tool or not. 
% The positive class is to use the tool. We measure precision and recall, and report the \emph{usability score (u)} which is the harmonic mean between them (f1-score).
% (2) \emph{Quality:} the model's ability to use a tool correctly (with the right parameters according to ground-truth). In the cases of \emph{adjust} and \emph{selective adjust} tools, we report the  \emph{quality score (q)} as the average \emph{cosine-similarity}. The cosine similarity is between the predicted vector of parameters and the ground-truth vector of parameters, where none of them is zero. In total, there are 14 parameters for adjust and 12 parameters for selective adjust. In the case of the \emph{filter} tool, the \emph{quality score (q)} is the \emph{accuracy}, defined as the proportion of correct predictions between the name of the predicted filter and the ground-truth filter (there are 23 available filters).
% Finally, we report the \emph{final score (f)} which is the harmonic mean between  \emph{usability score (u)} and \emph{quality score (q)}, as we want to achieve high performance on both, and hence we punish more for lower values.

% In addition to publish the results on \emph{All} distinct user's requests in the test-set, we analyze the performance on subsets of the test-set for more repeated (popular) user's requests. Let $r_i$  be distinct user's requests with at least $i$ calls. We publish the results on both $r_3$ and $r_5$.



% We also explore the impact on model performance when incorporating \emph{reasoning} as a component of the label, along with the values of the parameters. The reasoning should include a free text explanation of how to achieve the user's request by changing the parameters.
% The integration of intermediate reasoning steps, commonly referred to as Chain-of-Thought (CoT), has been observed to enhance the capability of LLMs in executing various tasks involving arithmetic, commonsense, and symbolic reasoning \cite{wei2022chain}. See Figure~\ref{fig:adjust_reasoning_example} for an example of the \emph{reasoning} and \emph{parameters' values} parts for the \emph{adjust} tool, given the ``golden hour'' user request. We can see that the actions outlined in the reasoning correspond with the adjustments made to the parameters.



% \noindent\textbf{Results.}
% Our results are summarized in Table~\ref{tab:eval_results}.
% \noindent\textbf{How does the use of smaller LLMs affect performance?}
% TODO



% \begin{table*}[!t]
% \centering
% \setlength{\tabcolsep}{2pt} 
% \begin{tabular}{c|c|ccc|ccc|ccc}
% \toprule
% \textbf{Model} & \multicolumn{1}{p{2cm}|}{\centering \textbf{Train} \\ \textbf{Size}} & \multicolumn{3}{c|}{\textbf{TestAll}} & \multicolumn{3}{c|}{\textbf{TestH3}} & \multicolumn{3}{c}{\textbf{TestH5}} \\
%  & & \textbf{A} & \textbf{SA} & \textbf{F} & \textbf{A} & \textbf{SA} & \textbf{F} & \textbf{A} & \textbf{SA} & \textbf{F} \\
% \midrule
% \multirow{9}{*}{LLaMA 2 (7B)} & \multirow{3}{*}{$\sim$8K} & - & - & - & - & - & - & - & - & - \\
%  & \multirow{3}{*}{$\sim$2K} & - & - & - & - & - & - & - & - & - \\
%  & \multirow{3}{*}{$\sim$1K} & \parbox{1cm}{.95\\ .54\\ .69} & - & \parbox{1cm}{.81\\ .64\\ .71} & \parbox{1cm}{.98\\ .55\\ .70} & - & \parbox{1cm}{.89\\ .60\\ .72} & \parbox{1cm}{.97\\ .59\\ \textbf{.74}} & - & \parbox{1cm}{.90\\ .72\\ \textbf{.80}} \\
% % Add the rest of your table content here
% \bottomrule
% \end{tabular}
% \caption{Pivoted Table Representation}
% \label{tab:pivoted_eval_results}
% \end{table*}









% \begin{table*}[!t]
%     \centering
%     \begin{tabular}{ccccccccc}
%         \toprule
%         \textbf{Model} & \textbf{\#Params} & \textbf{Evaluation Type} & \multicolumn{2}{c}{\textbf{Adjust}} & \multicolumn{2}{c}{\textbf{Selective Adjust}} & \multicolumn{2}{c}{\textbf{Filter}} \\
%         & & & u & q & u & q & u & q \\
%         \midrule
%         \multirow{2}{*}{LLaMA 2} & \multirow{2}{*}{7B} & Usability & 0.99  & 0.97 & 0.78 & 0.84 & 0.99 & 0.96 \\
%         & & Quality & 0.69  & \textbf{0.72} & 0.65 & \textbf{0.71} & 0.71 & 0.72 \\
%         \midrule
%         \midrule
        
%         \multirow{2}{*}{FlanT5-xl} & \multirow{2}{*}{3B} & Usability & -  & 0.98 & - & 0.8 & - & 0.98 \\
%         & & Quality & -  & 0.66 & - &  0.61 &  - & \textbf{0.78} \\
%         \midrule
%         \multirow{2}{*}{FlanT5-large} & \multirow{2}{*}{780M} & Usability & -  & 0.86 & - & 0.65 & - & 0.97 \\
%         & & Quality & -  & 0.65 & - &  0.51 &  - & 0.73 \\
%         \midrule
%         \multirow{2}{*}{FlanT5-base} & \multirow{2}{*}{250M} & Usability & -  & 1.0 & - & 0.83 & - & 0.97 \\
%         & & Quality & - & 0.61 & - & 0.51 & - & 0.73 \\
%         \midrule
%         \multirow{2}{*}{FlanT5-small} & \multirow{2}{*}{80M} & Usability & -  & 1.0 & - & 0.8 & - & 0.97 \\
%         & & Quality & - & 0.45 & - &0.33 & - & 0.68 \\
%         \bottomrule
%     \end{tabular}
%     \caption{TODO}
%     \label{tab:eval_results}
% \end{table*}


		
% Llama2 ckpt 60K 		
% flan-t5-base ckpt 55K
				


% \begin{table*}[!t]
%     \centering
%     \begin{tabular}{c| c | c|c|c|c}
%         \toprule
%         \textbf{Model} & \multicolumn{1}{p{2cm}|}{\centering \textbf{Train} \\ \textbf{Size}} & \textbf{Test} & \textbf{Adjust} & \textbf{Sel. Adjust} & \textbf{Filter} \\
%          \midrule
%         \multirow{6}{*}{LLaMA 2 (7B)} & $\sim$8K & All & (.95, .63, .76) & (.75, .66, .70) & (.81, .71, .76)  \\
%         & & $r_3$ &  (.98, .68, .80) &  (.82, .67, .74) &  (.92, .73, .81) \\
%         & & $r_5$ &  (.98, .75, \textbf{.85}) &  (.87, .71, \textbf{.78}) & (.91, .83, \textbf{.87}) \\
%         \cline{2-6}
%         & $\sim$2K & All & (.94, .59, .72) & (.68, .63, .66)  & (.60, .69, .64)\\
%         & & $r_3$ &  (.97, .64, .77) &  (.72, .63, .67)  & (.61, .70, .65) \\
%         & & $r_5$ & (.97, .71, \textbf{.82}) &  (.75, .67, \textbf{.71})  & (.65, .92, \textbf{.76}) \\
%         \cline{2-6}
%         & $\sim$1K & All & (.95, .54, .69) & (.64, .54, .58)  & (.81, .64, .71)\\
%         & & $r_3$ &  (.98, .55, .70) &  (.72, .51, .60)  & (.89, .60, .72) \\
%         & & $r_5$ & (.97, .59, \textbf{.74}) &  (.80, .54, \textbf{.64})  & (.90, .72, \textbf{.80}) \\
%         \midrule
%         \multirow{6}{*}{FlanT5-base (250M)} & $\sim$8K & All & (.95, .61, .74) & (.73, .66, .69) & (.81, .69, .75) \\
%         & & $r_3$ &  (.99, .64, .77) & (.81, .67, .73)  & (.90, .72, .80) \\
%         & & $r_5$ &  (.99, .74, \textbf{.85})	 & (.83, .75, \textbf{.79})  &(.93, .76, \textbf{.84}) \\
%         \cline{2-6}
%         & $\sim$2K & All & (.95, .56, .71) & (.70, .57, .63)  & (.75, .64, .69) \\
%         & & $r_3$ &  (.98, .58, .73) &  (.76, .56, .65) & (.84, .69, .76) \\
%         & & $r_5$ &  (.98, .64, \textbf{.78}) & (.76, .57, \textbf{.66})  & (.87, .73, \textbf{.79}) \\
%         \cline{2-6}
%         & $\sim$1K & All & (.95, .47, .63) & (.64, .31, .42)  & (.77, .60, .68)\\
%         & & $r_3$ &  (.99, .45, .62) & (.76, .29, .42)  & (.87, .57, .69) \\
%         & & $r_5$ &  (.99, .55, \textbf{.71}) & (.83, .30, \textbf{.45})  & (.88, .60, \textbf{.71}) \\
%         \midrule
%     \end{tabular}
%     \caption{(usability score, quality score, final score)}
%     \label{tab:eval_results}
% \end{table*}



















 % \multirow{6}{*}{FlanT5-base (250M)} & $\sim$8K & All & (.95, .62, .75) & (.73, .65, .69) & (.80, .72, .76)\\
 %        & & $h_3 &  (.99, .66, .79) & (.80, .65, .72)  & (.89, .74, .81) \\
 %        & & $h_5 &  (1.0, .75, \textbf{.85}) & (.87, .71, \textbf{.78})  & (.92, .76, \textbf{.83}) \\
 %        \cline{2-12}
 %        & $\sim$2K & All & .95 & .56 & .71 & .70 &  .57 &  .63  & .75 &  .64 &  .69\\
 %        & & $h_3 &  .98 & .58 & .73 & .76 &  .56 &  .65  & .84 & .69 &  .76 \\
 %        & & $h_5 &  .98 & .64 & \textbf{.78} & .76 &  .57 &  \textbf{.66}  & .87 &  .73 &  \textbf{.79} \\
 %        \cline{2-12}
 %        & $\sim$1K & All & .95 & .47 & .63 & .64 &  .31 &  .42  & .77 &  .60 &  .68\\
 %        & & $h_3 &  .99 & .45 & .62 & .76 &  .29 &  .42  & .87 &  .57 &  .69 \\
 %        & & $h_5 &  .99 & .55 & \textbf{.71} & .83 &  .30 &  \textbf{.45}  & .88 &  .60 &  \textbf{.71} \\





% \begin{table*}[!t]
% \centering
% \begin{tabular}{c|c|ccc|ccc|ccc}
% \toprule
% \textbf{Model} & \textbf{Train Size} & \multicolumn{3}{c|}{\textbf{TestAll}} & \multicolumn{3}{c|}{\textbf{TestH3}} & \multicolumn{3}{c}{\textbf{TestH5}} \\
%  & & \textbf{Adjust} & \textbf{Sel. Adjust} & \textbf{Filter} & \textbf{Adjust} & \textbf{Sel. Adjust} & \textbf{Filter} & \textbf{Adjust} & \textbf{Sel. Adjust} & \textbf{Filter} \\
% \midrule
% \multirow{3}{*}{LLaMA 2 (7B)} & $\sim$8K & - & - & - & - & - & - & - & - & - \\
%  & $\sim$2K & - & - & - & - & - & - & - & - & - \\
%  & $\sim$1K & .95, .54, .69 & - & .81, .64, .71 & .98, .55, .70 & - & .89, .60, .72 & .97, .59, \textbf{.74} & - & .90, .72, \textbf{.80} \\
% \midrule
% \multirow{3}{*}{FlanT5-base (250M)} & $\sim$8K & .95, .62, .75 & .73, .65, .69 & .80, .72, .76 & .99, .66, .79 & .80, .65, .72 & .89, .74, .81 & 1.0, .75, \textbf{.85} & .87, .71, \textbf{.78} & .92, .76, \textbf{.83} \\
% \bottomrule
% \end{tabular}
% \caption{Pivoted Table Representation}
% \label{tab:pivoted_eval_results}
% \end{table*}







a
